The complexity of soundness in workflow nets

Workflow nets are a popular variant of Petri nets that allow for algorithmic formal analysis of business processes. The central decision problems concerning workflow nets deal with soundness, where the initial and final configurations are specified. Intuitively, soundness states that from every reachable configuration one can reach the final configuration. We settle the widely open complexity of the three main variants of soundness: classical, structural and generalised soundness. The first two are EXPSPACE-complete, and, surprisingly, the latter is PSPACE-complete, thus computationally simpler.

==> figures/arc_weights_binary.tex <==
\begin{tikzpicture}
    \node[place, label=below:$p$] (p) {};

    \node[transition, right=1cm of p, label=below:$t$] (t) {};

    \node[place, right=1cm of t, label=below:$q$] (q) {};

    \path[->]
    (p) edge[]            node[above] {$2$}           (t)
    (t) edge[]            node[above] {$2$}           (q);
\end{tikzpicture}
